Balancing Isolation and Sharing of Data for Third-Party Extensible App Ecosystems

In the landscape of application ecosystems, today's cloud users wish to personalize not only their browsers with various extensions or their smartphones with various applications, but also the various extensions and applications themselves. The resulting personalization significantly raises the attractiveness for typical Web 2.0 users, but gives rise to various security risks and privacy concerns, such as unforeseen access to certain critical components, undesired information flow of personal information to untrusted applications, or emerging attack surfaces that were not possible before a personalization has taken place. In this paper, we propose a novel extensibility mechanism which is used for implementing personalization of existing cloud applications towards (possibly untrusted) components in a secure and privacy-friendly manner. Our model provides a clean component abstraction, thereby in particular ruling out undesired component accesses and ensuring that no undesired information flow takes place between application components -- either trusted from the base application or untrusted from various extensions. We then instantiate our model in the SAFE web application framework (WWW 2012), resulting in a novel methodology that is inspired by traditional access control and specifically designed for the newly emerging needs of extensibility in application ecosystems. We illustrate the convenient usage of our techniques by showing how to securely extend an existing social network application.

==> Makefile <==
MAIN = main

$(MAIN).pdf: $(MAIN).ps
	ps2pdf $< $@

mate:
	pdflatex -synctex=1 $(MAIN)

$(MAIN).ps: $(MAIN).dvi
	dvips -t letter $<

$(MAIN).dvi: $(MAIN).tex tex/* src/* res/*
	latex -halt-on-error -synctex=1 $(MAIN)
	-bibtex -terse $(MAIN)
	latex -synctex=1 $(MAIN) > /dev/null
	latex -synctex=1 $(MAIN) > /dev/null

.PHONY: clean

clean:
	-find . \( -name "*.log" -o -name "*.aux" -o -name "*.bbl" -o -name "*.blg" -o -name "*.out" \) -exec rm {} \;
	-rm -f $(MAIN).pdf $(MAIN).ps $(MAIN).dvi $(MAIN).synctex.gz


==> tex/extended_abstract.tex <==
[Extended Abstract]


==> tex/scratchboard.tex <==
\section{Scratchboard}

  Formal Model Notes:
  \begin{itemize}
    \item Our definition of $\mathit{req\_valid}$ requires \emph{all} affected principals of \emph{every} dimension to approve a request on shared data.
    \item Further checks on $r$ are out of the policies' scope, e.g., whether the operation implied by $r$ is permissive at all.
    \item This definition does not consider recursion (transitive sharing).
    \item $\mathit{sh_{\cP_i}(\cdot, \cdot, \cdot)}$ must be ``honest''. Maybe, a metric for that could be $\mathit{pol(r, u', c')}$.
    \item A recursive definition of $\mathit{pol(\cdot, \cdot, \cdot)}$ might be advisable.
    \item Which $\mathit{aff(r_{t+1})}$ information is assumed if it accesses a shared dataset created by $\mathit{aff(r_{t})}$?
  \end{itemize}

  Formal Model Todos:
  \begin{itemize}
    \item leverage the intersection dimensions as necessary condition
    for data access. Example: smartphone with unauthenticated user / locked
    screen. At this point, no component/app shall have access to any
    user-related data.
  \end{itemize}

  Instantiation Todos:
  \begin{itemize}
    \item How do we force input tables to provide proper owner information? Currently, output tables can specify
    arbitrary values for the owner column.
  \end{itemize}

  Implementation Todos:
  \begin{itemize}
    \item Invariants on local tables
  \end{itemize}

\subsection{Soundness of the Instantiation}

  We claim now that $\mathit{sb(r, u, c)} \Rightarrow \mathit{req\_valid(r, u, c)}$ -- i.e., that the sandbox is at least restrictive as the presented formal model.
  From the particular parts of $\mathit{sb}$ and using our instantiations, we can derive:
  \begin{flalign*}
    \text{(A)}\; & \forall t \in \mathit{scope_{\cT}(r)} \colon t \in \mathit{lt(c)} \Rightarrow_{(\ref{eq:local_funit_owner})} &\\
                 & \forall t \in \mathit{scope_{\cT}(r)} \colon \forall d \in \mathit{data(t)} \colon \mathit{aff_{\cC}(d)} = c \Rightarrow_{(\ref{eq:data_table_completeness})} &\\
                 & \forall d \in \mathit{scope_{\cD}(r)} \colon \mathit{aff_{\cC}(d)} = c &\\
    \text{(B)}\; & \forall d \in \mathit{scope_{\cD}(r)} \colon \mathit{own(d)} = u \Rightarrow_{(\ref{eq:owner_is_affected_user})} &\\
                 & \forall d \in \mathit{scope_{\cD}(r)} \colon \mathit{aff_{\cU}(d)} = u &\\
    \text{(D)}\; & t \in \mathit{lt(c)} \Rightarrow_{(\ref{eq:local_funit_owner})} &\\
                 & \forall d \in \mathit{data(t)} \colon \mathit{aff_{\cC}(d)} = c &\\
    \text{(D)}\; & t \in \mathit{lt(c)} \Rightarrow_{(\ref{eq:local_is_public})} &\\
                 & \forall d \in \mathit{data(t)} \colon \mathit{own(d)} = u \vee \mathit{sh_{\cU}(own(d), u, d)} \Rightarrow_{(\ref{eq:owner_is_affected_user})} &\\
                 & \forall d \in \mathit{data(t)} \colon \mathit{aff_{\cU}(d)} = u \vee \mathit{sh_{\cU}(aff_{\cU}(d), u, d)} &\\
    \text{(E)}\; & t \in \mathit{it(c, u)} \Rightarrow_{(\ref{eq:itable_unit_sharing})} &\\
                 & \forall d \in \mathit{data(t)} \colon \mathit{sh_{\cC}(src(d), c, d)} \Rightarrow_{(\ref{eq:itable_affected_unit})} &\\
                 & \forall d \in \mathit{data(t)} \colon \mathit{sh_{\cC}(aff_{\cC}(d), c, d)} &\\
    \text{(E)}\; & t \in \mathit{it(c, u)} \Rightarrow_{(\ref{eq:input_is_public})} &\\
                 & \forall d \in \mathit{data(t)} \colon \mathit{own(d)} = u \vee \mathit{sh_{\cU}(own(d), u, d)} \Rightarrow_{(\ref{eq:owner_is_affected_user})} &\\
                 & \forall d \in \mathit{data(t)} \colon \mathit{aff_{\cU}(d)} = u \vee \mathit{sh_{\cU}(aff_{\cU}(d), u, d)} &
  \end{flalign*}
  We can thus replace the overall implications
  \begin{equation*}
    \begin{alignedat}{3}
      &\text{(A)}\leadsto\; & \forall d \in \mathit{scope_{\cD}(r)} \colon & \mathit{aff_{\cC}(d)} = c &\\
      &\text{(B)}\leadsto\; & \forall d \in \mathit{scope_{\cD}(r)} \colon & \mathit{aff_{\cU}(d)} = u &\\
      &\text{(D)}\leadsto\; & \forall d \in \mathit{data(t)} \colon      & \mathit{aff_{\cC}(d)} = c \:\wedge &\\
      &                     &                                            & (\mathit{aff_{\cU}(d)} = u \vee \mathit{sh_{\cU}(aff_{\cU}(d), u, d)}) &\\
      &\text{(E)}\leadsto\; & \forall d \in \mathit{data(t)} \colon      & \mathit{sh_{\cC}(aff_{\cC}(d), c, d)} \:\wedge &\\
      &                     &                                            & (\mathit{aff_{\cU}(d)} = u \vee \mathit{sh_{\cU}(aff_{\cU}(d), u, d)}) &
    \end{alignedat}
  \end{equation*}
  in the $\mathit{sb(r, u, c)}$ definition -- the outcome shall satisfy our claim and thus the formal model.

  By the implications of (D) and (E), we can derive the overall semantics of (C), i.e., of a \texttt{SEL} operation:
  \begin{equation}\label{sb_read}
    \begin{alignedat}{3}
      &                                                  && \text{(C)}                                 && \\
      & \Leftrightarrow                                  && \forall t \in \mathit{scope_{\cT}(r)} \colon && \text{(D)} \vee \text{(E)} \\
      & \Rightarrow_{(\ref{eq:data_table_completeness})} && \forall d \in \mathit{scope_{\cD}(r)} \colon && (\mathit{aff_{\cC}(d)} = c \vee \mathit{sh_{\cC}(aff_{\cC}(d), c, d)}) \:\wedge\\
      &                                                  &&                                            && (\mathit{aff_{\cU}(d)} = u \vee \mathit{sh_{\cU}(aff_{\cU}(d), u, d)})
    \end{alignedat}
  \end{equation}
  Furthermore, for a request being an \texttt{INS}, \texttt{UPD}, or \texttt{DEL} operation, we have:
  \begin{equation}\label{sb_write}
    \begin{aligned}
                        & \text{(A)} \:\wedge\: \text{(B)} \\
      \Leftrightarrow\; & \forall d \in \mathit{scope_{\cD}(r)} \colon \mathit{aff_{\cC}(d)} = c \:\wedge\: \mathit{aff_{\cU}(d)} = u
    \end{aligned}
  \end{equation}
  If we reconsider the formal model as in \autoref{eq:req_valid}, the instantiation to the $\langle \cU, \cC \rangle$ universe gives:
  \begin{align*}%{eq:req_valid}
    \mathit{req\_valid(r, u, c)} \mapsto\: & \forall d \in \mathit{scope_{\cD}(r)}\colon \\
                                           & (\mathit{aff_{\cU}(d)} = u \vee \mathit{sh_{\cU}(aff_{\cU}(d), u, d)}) \:\wedge \\
                                           & (\mathit{aff_{\cC}(d)} = c \vee \mathit{sh_{\cC}(aff_{\cC}(d), c, d)})
  \end{align*}
  Both branches of our sandbox $\mathit{sb}$, i.e., \eqref{sb_read} and \eqref{sb_write}, reflect that for every dimension, either own or explicitly shared datasets are affected -- and thus satisfy the formal model. \hfill $\Box$

